Adaptive Hierarchical Clustering Using Ordinal Queries

In many applications of clustering (for example, ontologies or clusterings of animal or plant species), hierarchical clusterings are more descriptive than a flat clustering. A hierarchical clustering over $n$ elements is represented by a rooted binary tree with $n$ leaves, each corresponding to one element. The subtrees rooted at interior nodes capture the clusters. In this paper, we study active learning of a hierarchical clustering using only ordinal queries. An ordinal query consists of a set of three elements, and the response to a query reveals the two elements (among the three elements in the query) which are "closer" to each other than to the third one. We say that elements $x$ and $x'$ are closer to each other than $x"$ if there exists a cluster containing $x$ and $x'$, but not $x"$. When all the query responses are correct, there is a deterministic algorithm that learns the underlying hierarchical clustering using at most $n \log_2 n$ adaptive ordinal queries. We generalize this algorithm to be robust in a model in which each query response is correct independently with probability $p > \frac{1}{2}$, and adversarially incorrect with probability $1 - p$. We show that in the presence of noise, our algorithm outputs the correct hierarchical clustering with probability at least $1 - \delta$, using $O(n \log n + n \log(1/\delta))$ adaptive ordinal queries. For our results, adaptivity is crucial: we prove that even in the absence of noise, every non-adaptive algorithm requires $\Omega(n^3)$ ordinal queries in the worst case.

==> resources/simulate-query.tex <==
%\section{The formal specification of the algortihm \SimulateVertexQuery}
%\label{sec:simulate-query}

\InsertAlgorithm{\SimulateVertexQuery $(\Tree, \Vertex, \ElS)$}{alg:simulate}{
\IF{\Vertex is the root of \Tree}
\STATE{Make one ordinal query for \ElS with pivot \Vertex, and return its
  result.}
\STATE{(Since $\Subtree{\Vertex} = \Set{\Vertex}$ in this case, the
  response reveals the root as the proposed answer.)}
\ELSIF{\Vertex is a leaf}
\STATE{Let \VertexP be the parent of \Vertex in \Tree.}
\STATE{Make one ordinal query for \ElS with pivot \VertexP.}
\IF{the response places \ElS at \Vertex}
\RETURN{the vertex \Vertex as a proposed answer.}
\ELSE
\RETURN{the direction towards \VertexP.}
\ENDIF
\ELSE
\STATE{Let \VertexP be the parent of \Vertex in \Tree.}
\STATE{Let $k_p$ be a sufficiently large (odd) constant.}
\STATE{Make $k_p$ ordinal queries for \ElS with pivot \Vertex.}
\IF{a strict majority of responses place \ElS in \Subtree[L]{\Vertex}}
\RETURN{the direction towards the left child of \Vertex}
\ELSIF{a strict majority of responses place \ElS in \Subtree[R]{\Vertex}}
\RETURN{the direction towards the right child of \Vertex}
\ELSIF{a strict majority of responses place \ElS in \Subtree{\Vertex}}
\STATE{Make $k_p$ ordinal queries for \ElS with pivot \VertexP.}
\IF{a strict majority of responses place \ElS in the subtree of
  \VertexP containing \Vertex}
\RETURN{the vertex \Vertex as a proposed answer.}
\ELSIF{a strict majority of responses place \ElS in \Subtree{\VertexP}}
\RETURN{the direction towards \VertexP.}
\ELSIF{a strict majority of responses place \ElS in the other subtree
  of \VertexP}
\RETURN{the direction towards \VertexP.}
\ELSE
\RETURN{an arbitrary response.}
\ENDIF
\ELSE
\RETURN{an arbitrary response.}
\ENDIF
\ENDIF
}

